Low-Cost High-Power Membership Inference Attacks

Membership inference attacks aim to detect if a particular data point was used in training a model. We design a novel statistical test to perform robust membership inference attacks (RMIA) with low computational overhead. We achieve this by a fine-grained modeling of the null hypothesis in our likelihood ratio tests, and effectively leveraging both reference models and reference population data samples. RMIA has superior test power compared with prior methods, throughout the TPR-FPR curve (even at extremely low FPR, as low as 0). Under computational constraints, where only a limited number of pre-trained reference models (as few as 1) are available, and also when we vary other elements of the attack (e.g., data distribution), our method performs exceptionally well, unlike prior attacks that approach random guessing. RMIA lays the groundwork for practical yet accurate data privacy risk assessment in machine learning.

==> figure_scripts/distributions_non_members.tex <==
\begin{figure*}[h]
    \centering
      \includegraphics[width=0.42\linewidth]{fig/distributions/cifar10.png}\hspace*{2em}
      \includegraphics[width=0.42\linewidth]{fig/distributions/cifar100.png}\vspace*{2em}
      \includegraphics[width=0.42\linewidth]{fig/distributions/cinic10.png}\hspace*{2em}
      \includegraphics[width=0.42\linewidth]{fig/distributions/purchase100.png}
      \caption{Distributions of average prediction probability for non-member samples across trained models. For each dataset, we train 254 models with half of the dataset randomly selected as the training set. Then, we calculate the average prediction probability for non-member samples in each model and illustrate the distribution of these probabilities across all models. The x-axis represents the average prediction probability (within each model), while the y-axis denotes the number of models.}      \label{fig:prob_distribution_non_members_across_models}
  \end{figure*}
